QR2: A Third-party Query Reranking Service Over Web Databases

The ranked retrieval model has rapidly become the de-facto way for search query processing in web databases. Despite the extensive efforts on designing better ranking mechanisms, in practice, many such databases fail to address the diverse and sometimes contradicting preferences of users. In this paper, we present QR2, a third-party service that uses nothing but the public search interface of a web database and enables the on-the-fly processing of queries with any user-specified ranking functions, no matter if the ranking function is supported by the database or not.

==> arch.tex <==
\section{Architecture}\label{sec:arch}

\begin{figure}[t]
	\centering
	\includegraphics[width=0.48\textwidth]{img/architecture.png}
	\vspace{-3mm}
	\caption{\small Architecture of Q2R.}
	\vspace{-2mm}
	\label{fig:architecture}
\end{figure}

The web service in the architecture is the main orchestrator behind the whole system. The user connects to the web service via the internet and gives the choice of which service the user wants to use (e.g. Google flights, Bluenile, Zillow etc). The web server then creates a session for the user and processes the user’s ranking and filtering query and constructs the best set of queries to efficiently get the results from the Top-k query interface (e.g. Google flights, Bluenile, Zillow etc) re-rank it and present the results to the user. A cache is used for every user, since retaining a cache fastens the query processing and subsequent get-next operations can be done faster. A mysql database is used in our system to store the dense region cache, since the retrival of results from a dense region of tuples becomes very expensive (in terms of the number of queries). We deploy a dense region cache to counter this problem. We frequently update the dense region cache to maintain its consistancy with the Top-k interface. Another frequent question that gets asked is that how does the system handle cases where the number of queries exceeds the limit on the number of queries on the backend database can get from a single user (due to security measure). Since the algorithms MD-index and MD-binary are desinged in such a way to use least amount of queries to query the Topk interface, realistically we not hit the limit for a few dozen users. In that case, we could use a distributed system to spread out the query processing across different servers.
